Approximate Inference with Amortised MCMC

We propose a novel approximate inference algorithm that approximates a target distribution by amortising the dynamics of a user-selected MCMC sampler. The idea is to initialise MCMC using samples from an approximation network, apply the MCMC operator to improve these samples, and finally use the samples to update the approximation network thereby improving its quality. This provides a new generic framework for approximate inference, allowing us to deploy highly complex, or implicitly defined approximation families with intractable densities, including approximations produced by warping a source of randomness through a deep neural network. Experiments consider image modelling with deep generative models as a challenging test for the method. Deep models trained using amortised MCMC are shown to generate realistic looking samples as well as producing diverse imputations for images with regions of missing pixels.

==> divergence.tex <==

%\subsection{Adversarially Estimated Divergences}
\subsection{The choice of update rule}
The choice of the update signal and ways to estimate it plays a crucial role in our framework, 
and it should be carefully selected to ensure both strong discrimination power and 
computational tractability with respect to the parametric family of $q$ that we use. 
We discuss three update rules in the following.
%It is crucial that the divergence/discrepancy measure $\mathrm{D}[ \cdot || \cdot ]$ is carefully selected based on the knowledge of posterior shape and the design of $q$. 
%
\paragraph{KL divergence minimisation} A simple approach would minimise the inclusive KL-divergence
$$\mathrm{D}_{\text{KL}}[q_T||q] = \mathbb{E}_{q_T} \left[ \log q_T(\bm{z}|\bm{x}) - \log q(\bm{z}|\bm{x}) \right],$$
and using the projection-based method it only requires an MC estimate of $-\mathbb{E}_{q_T}[\log q(\bm{z}|\bm{x})]$. 
This gives a simple algorithm that is a hybrid of MCMC and VI, and appears to be new to our knowledge. Similar algorithms include the so called cross entropy method \citep{crossentrode2005tutorial} which replaces $q_T$ with an importance weighted distribution, and methods for tuning proposal distributions for SMC \cite{cornebise:smc2009,gu:nasmc2015}.
%
\paragraph{Adversarially estimated divergences} 
Unfortunately, the inclusive KL divergence requires the $q$ density to be computable, 
therefore it cannot be used directly for wild  approximations.
In such cases we assume that we have access to both $q$ and $q_T$ only through samples $\{\bm z_0^k\}\sim q(\bm z | \bm x)$ and $\{\bm z_T^k\}\sim q_T(\bm z | \bm x) $, and we need to estimate the divergence based on the two samples. 
%
To address this, we borrow the 
%One of the most powerful way to achieve this is  using  
idea of generative adversarial networks (GAN) \cite{goodfellow:gan2014} to construct a sample-based estimator of the selected divergence. As an example, consider the Jensen-Shannon divergence:
$
\mathrm{D}_{\text{JS}}[q_T||q] = \frac{1}{2} \mathrm{D}_{\text{KL}}[q_T || \tilde{q}] + \frac{1}{2} \mathrm{D}_{\text{KL}}[q || \tilde{q}],
$
with $\tilde{q} = \frac{1}{2} q + \frac{1}{2} q_T$.
Since none of the three distributions have tractable density, a discriminator $d_{\bm{\psi}}(\bm{z}|\bm{x})$ is trained to provide a stochastic lower-bound 
\begin{equation}
\mathrm{D}_{\text{JS}}[q_T||q] \geq \mathrm{D}_{\text{adv}}[\{\bm{z}_T^k \} || \{ \bm{z}_0^k \} ] = \frac{1}{K} \sum_{k=1}^K \log \sigma(d_{\bm{\psi}}(\bm{z}_T^k | \bm{x}))
+ \frac{1}{K} \sum_{k=1}^K \log (1 - \sigma(d_{\bm{\psi}}(\bm{z}_0^k | \bm{x}))),
\label{eq:gan_objective}
\end{equation}
with $\sigma(\cdot)$ the sigmoid function and $\bm{z}_0^k$, $\bm{z}_T^k$ samples from $q$ and $q_T$, respectively. 
%
Recent work \cite{nowozin:fgan2016} extends adversarial training to $f$-divergences where the two KL-divergences are special cases in that rich family. In such case $\mathrm{D}_{\text{adv}}$ also corresponds to the variational lower-bound to the selected $f$-divergence and the discriminator can also be defined accordingly. Furthermore, density ratio estimation literature \cite{nguyen2010estimating, sugiyama:ratio2009,sugiyama:ratio2012} suggests that the discriminator $d_{\bm{\psi}}$ in (\ref{eq:gan_objective}) can be used as an estimator of $\log \frac{q_T}{q}$, i.e.~the objective function for $q$ could be decoupled from that for the discriminator \cite{mohamed:gan2016}.

\paragraph{Energy matching} 
An alternative approach to achieve $q_T \approx q$ would match the first $M$ moments between $q_T$ and $q$, an in particular matching the mean and variance is equivalent to minimising $\mathrm{D}_{\text{KL}}[q_T || q]$ with $q_T$ fixed and $q$ a Gaussian distribution. However it is difficult to know beforehand which moments are important for accurate approximations. Instead we propose \emph{energy matching}, which matches the expectation of the log joint distribution $\log p(\bm{x}, \bm{z})$ under $q$ and $q_T$:
\begin{equation}
\min_{\vparam} \mathcal{F}(\vparam) = \big| \mathbb{E}_{q_T(\bm{z}_T|\bm{x})}\left[ \log p(\bm{x}, \bm{z}_T) \right] - \mathbb{E}_{q_{\vparam}(\bm{z}|\bm{x})}\left[ \log p(\bm{x}, \bm{z}) \right] \big|^{\beta}, \quad \beta > 0,
\label{eq:energy_matching}
\end{equation} 
%
Though $\mathcal{F}$ is not a divergence/discrepancy measure between $q$ and $q_T$, we argue that this construction would encourage the method to match moments that are more effective for accurate predictive distribution approximation, which is still good for inference. Furthermore, as (\ref{eq:energy_matching}) can be approximated with Monte Carlo methods which only require samples from $q(\bm{z}|\bm{x})$, this energy matching objective can be applied to wild variational inference settings as it does not require density evaluation of $q$. We provide another motivation for energy matching by considering contrastive divergence \citep{hinton:cd2002} as follows. First since $\Delta_{\text{CD}} := \mathrm{KL}[q||p] - \mathrm{KL}[q_T||p] \geq 0$, it can be used as a minimisation objective to fit an approximate posterior $q$. Expanding this contrastive divergence equation, we have:
\begin{equation}
\begin{aligned}
\Delta_{\text{CD}} &= \mathbb{E}_{q(\bm{z}|\bm{x})} \left[ \log \frac{q(\bm{z}|\bm{x})}{p(\bm{x}, \bm{z})}  \right] - \mathbb{E}_{q_T(\bm{z}_T|\bm{x})} \left[ \log \frac{q_T(\bm{z}_T|\bm{x})}{p(\bm{x}, \bm{z}_T)}  \right] \\
	&= \mathbb{E}_{q_T(\bm{z}_T|\bm{x})} \left[ \log p(\bm{x}, \bm{z}_T)  \right] - \mathbb{E}_{q(\bm{z}|\bm{x})} \left[ \log p(\bm{x}, \bm{z})  \right] + \mathbb{E}_{q(\bm{z}|\bm{x}) \mathcal{K}_T(\bm{z}_T | \bm{z})} \left[ \log \frac{ q_T(\bm{z} | \bm{z}_T, \bm{x})}{\mathcal{K}_T(\bm{z}_T | \bm{z})} \right],
\end{aligned}
\label{eq:cd}
\end{equation}
where $q_T(\bm{z} | \bm{z}_T, \bm{x}) = q(\bm{z}|\bm{x}) \mathcal{K}_T(\bm{z}_T|\bm{z}) / q_T(\bm{z}_T|\bm{x})$ is the ``posterior'' of $\bm{z}$ given the sample $\bm{z}_T$ after T-step MCMC. We ignore the third term in (\ref{eq:cd}) when $T$ is small as now $\z$ and $\z_T$ are highly correlated, which motivates the energy matching objective (\ref{eq:energy_matching}). For large $T$ one can also use density ratio estimations methods to estimate the third term, but we leave the investigation to future work.

\section{Approximate MLE with amortised MCMC}
Learning latent variable models has become an important research topic with increasing interest. These models are optimised using approximate maximum likelihood (MLE), with the latent variables being inferred during training.
%
Current practices often maximise the variational lower-bound:
\begin{equation}
\mathbb{E}_q \left[ \log p(\bm{x} | \bm{z}; \bm{\theta}) \right] - \mathrm{D}_{\text{KL}}[q(\bm{z}|\bm{x})||p_0(\bm{z})]
= \log p(\bm{x}|\bm{\theta}) - \mathrm{D}_{\text{KL}}[q(\bm{z}|\bm{x}) || p(\bm{z}| \bm{x}, \bm{\theta}) ].
\label{eq:vae_mle}
\end{equation}
%
As a by-product of the proposed amortisation framework, we discuss approximate MLE with MCMC samples in the generative modelling context.
%
Again because $\mathrm{D}_{\text{KL}}[q || p] \geq \mathrm{D}_{\text{KL}}[q_T || p]$ if $p$ is the stationary distribution of the Markov chain, the following objective
\begin{equation}
\log p(\bm{x}|\bm{\theta}) - \mathrm{D}_{\text{KL}}[q_T(\bm{z}|\bm{x}) || p(\bm{z}| \bm{x}, \bm{\theta}) ]
\label{eq:mcmc_mle}
\end{equation}
forms a tighter lower-bound to the marginal likelihood. Empirical evidences \cite{burda:iwae2016,li:vrbound2016} suggested tighter lower-bounds often lead to better results. Moreover, optimising (\ref{eq:mcmc_mle}) w.r.t.~$\bm{\theta}$ only requires computing 
$\mathbb{E}_{q_T}[ \log p(\bm{x} | \bm{z}, \bm{\theta}) ] \approx \frac{1}{K} \sum_k \log p(\bm{x} | \bm{z}_T^k, \bm{\theta}) $
 with samples $\bm{z}_T^k \sim q_T$ from the Markov chain initialised at $q$, hence density evaluation of $q_T$ is not needed. This is especially desirable at the early stage of learning, as the $q$ distribution is still far away from the exact posterior.

Now we turn to the algorithmic design for optimising $q$ as the initial proposal. A naive approach would maximise the variational lower-bound (\ref{eq:vae_mle}) w.r.t.~$\bm{\phi}$ if the density is tractable. These white-box proposals could also be learned with amortised MCMC, if the inclusive KL divergence is selected. In the case where the approximate posterior is wild, we train another discriminator $d_{\bm{\psi}}$ to estimate the selected divergence, and propagate learning signals back through the samples from $q$.
%
The full method is presented in Algorithm \ref{alg:amortised_mcmc_adversarial}. Note here the update step for the discriminator and the $q$ distribution could be executed for more iterations in order to achieve better approximations to the current posterior. This strategy turns the algorithm into a stochastic EM procedure with MCMC methods approximating the E-step \cite{celeux:sem1985,celeux:sem1995}. Two-sample based techniques, such as kernel maximum mean discrepancy (MMD) \cite{gretton:mmd2012}, can also be applied as the discrepancy measure in step 3, but this is not explored here. 

%and clearly this avoids the usage of a discriminator and unstable adversarial learning. %However computing an accurate empirical estimate $\mathrm{\hat{D}}[q_T||q]$ of MMD requires many samples from both distributions, and the number of samples required grows with the dimensionality of the latent variable $\bm{z}$. Furthermore, in general we need to simulate $2K$ parallel Markov chains to remove the correlation between samples of $\bm{z}_T$ and $\bm{z}_0$, which brings in prohibitive cost for tasks like training deep generative models. We continue discussing this correlation issue in the appendix, and in the experiments we only consider $\bm{z}_T^k$ generated by a Markov chain started at $\bm{z}_0^k$.

%%% algorithm %%%
\begin{algorithm}[t] 
\begin{algorithmic}[1] 
	\STATE sample $\bm{z}_{0}^{1}, ..., \bm{z}_{0}^K \sim q_{\bm{\phi}}(\bm{z}|\bm{x})$, and simulate $\bm{z}_{T}^{k} \sim \mathcal K_T(\cdot |\bm{z}_{k}^{0} )$.	 
	\STATE compute $\mathrm{D}_{\text{adv}}[ \{ \bm{z}_T^k \}  || \{ \bm{z}_0^k \} ]$ using discriminator $\bm\psi$.
	\STATE update $\bm{\phi}$ and $\bm{\psi}$ by 1-step gradient descent/ascent.
	\STATE if learning $\bm{\theta}$: compute 1-step gradient ascent with
	$ \nabla_{\bm{\theta}} \frac{1}{K} \sum_{k=1}^K \log p(\bm{\bm{x}} | \bm{z}_T^k, \bm{\theta}).$
\end{algorithmic}
\caption{Amortised MCMC with adversarially estimated divergences (one update iteration)}
\label{alg:amortised_mcmc_adversarial} 
\end{algorithm}

%%% algorithm %%%

%We also briefly discuss the effect of the Markov chain length $T$ on the approximation quality, in the context of using adversarially estimated divergences. In theory, even when selecting $T=1$, minimising $\mathrm{D}[q_1||q]$ would return the exact approximation if $q$ is sufficiently flexible to capture the exact posterior. However in practice using small $T$ introduces strong correlations between $\bm{z}$ and $\bm{z}_T$, hence the discriminator could be easily fooled, and the learning signal provided by the estimated divergence will be too weak, especially for a flexible $q$ distribution to learn the posterior landscape (e.g.~those produced using neural networks with stochastic inputs). Though this could potentially be avoided by using uncorrelated $\bm{z}$ and $\bm{z}_T$, but again it is computationally too expensive for the tasks we consider. 
